The Gaia-ESO Survey: Constraining evolutionary models and ages for young low mass stars with measurements of lithium depletion and rotation

A growing disquiet has emerged in recent years that standard stellar models are at odds with observations of the colour-magnitude diagrams (CMDs) and lithium depletion patterns of pre main sequence (PMS) stars in clusters. In this work we select 1,246 high probability K/M-type constituent members of 5 young open clusters (5--125\,Myr) in the Gaia-ESO Survey to test a series of models that use standard input physics and others that incorporate surface magnetic fields or cool starspots. We find that: standard models provide systematically under-luminous isochrones for low-mass stars in the CMD and fail to predict Li-depletion of the right strength at the right colour; magnetic models provide better CMD fits with isochrones that are $\sim 1.5-2$ times older, and provide better matches to Li depletion patterns. We investigate how rotation periods, most of which are determined here for the first time from Transiting Exoplanet Survey Satellite data, correlate with CMD position and Li. Among the K-stars in the older clusters we find the brightest and least Li-depleted are the fastest rotators, demonstrating the classic "Li-rotation connection" for the first time at $\sim 35$ Myr in NGC 2547, and finding some evidence that it exists in the early M-stars of NGC 2264 at $<10\,$Myr. However, the wide dispersion in Li depletion observed in fully-convective M-dwarfs in the $\gamma$ Vel cluster at $\sim 20$ Myr appears not to be correlated with rotation and is challenging to explain without a very large ($>10$ Myr) age spread.

==> t2.tex <==
{\centering
\begin{table*}
\begin{center}
\begin{tabular}{lllllllll}
\hline
\hline
Name                     & $P_{\rm TESS}$    & Sector & $f_{\rm max}/f_{\rm FAP}$ & $f_{\rm max}/f_{2}$ & $\log (f_{\rm bg}/f_{*})$ & $P_{\rm lit}$ & $P_{\rm rot}$ & code  \\
(Gaia DR2-)              & (days)            &        &                           &                     &                           & (days)        & (days)        &       \\
\hline
1  & $5.142 \pm 0.424$ & 6 & $25.33$ &  $3.25$ & $+0.25$ &               & $5.142 \pm 0.424$ & 1 \\
2  & $2.444 \pm 0.090$ & 6 & $15.02$ &  $2.30$ & $+0.21$ &               & $2.443 \pm 0.090$ & 1 \\
3  & $5.734 \pm 0.539$ & 6 & $14.09$ &  $2.04$ & $-0.60$ & $5.550$, V+16 & $5.734 \pm 0.539$ & 3 \\
4  &                   &          &         &         &         &               &                   & 0 \\
5  &                   &          &         &         &         &               &                   & 0 \\
6  &                   &          &         &         &         &               &                   & 0 \\
7  & $3.728 \pm 0.220$ & 6 & $16.89$ &  $3.53$ & $-0.19$ &               & $3.728 \pm 0.220$ & 1 \\
8  & $0.858 \pm 0.012$ & 6 & $37.04$ & $13.22$ & $-0.37$ & $4.250$, V+16 & $0.858 \pm 0.012$ & 5 \\
9  &                   &          &         &         &         &               &                   & 0 \\
10 &                   &          &         &         &         &               &                   & 0 \\
\hline
\end{tabular}
\caption{Period data for the 1,\,093 objects in the sample. Column 1 is the source identifier from Gaia DR2. Columns 2--6 contain data from the TESS analysis in this work -- the calculated rotation period, TESS sector and the three threshold values described in $\S$\ref{S_TESS_Comparison}. Column 7 provides the literature rotation period and the reference. Column 8 is the final rotation period used in this analysis and column 9 denotes a code number describing how the final period was chosen. Only the first 10 sources are listed here. The entire table is available in electronic format. References: A+13 = \protect\cite{2013a_Affer}; I+07 = \protect\cite{2007a_Irwin}; I+08 = \protect\cite{2008a_Irwin}; L+04 = \protect\cite{2004a_Lamm}; M+04 = \protect\cite{2004a_Makidon}; V+16 = \protect\cite{2017a_Venuti}.}
\label{T_Periods}
\end{center}
\end{table*}}


==> t_CMD_StudentT.tex <==
{\centering
\begin{table}
\caption{Results for the statistical tests comparing the $P_{\rm rot}$ distributions between bright and faint samples in each spectral-type bin. Columns 3 and 4 indicate the number of objects in the bright and faint sample, respectively. The Student t-statistic in column 5 represents the difference in the means between the bright and faint populations, where the p-values (that they have significantly different means) are provided in parentheses. Column 6 gives the correlation coefficients (r-scores) for $P_{\rm rot}$ versus $\Delta G_0$ and corresponding p-values in parentheses. Only the bins with p-values $< 0.2$ from the t-scores are displayed and asterisks denote p-values that are at least 10 times smaller than 0.01 (highly significant).}
%1.13$e$-4, 3.55$e$-5, 2.2$e$-4, 0.001
\begin{center}
%\begin{tabular}{p{1.35cm}p{1.05cm}p{0.8cm}p{0.8cm}p{0.9cm}p{1.0cm}}
\begin{tabular}{p{1.35cm}p{1.05cm}p{0.40cm}p{0.40cm}p{1.30cm}p{1.40cm}}
\hline
\hline
Cluster & SpT bin & B     & F      & t-score  & r-score \\
\hline
%
$\lambda$ Ori & All M &  19 &  17 & $+1.54(0.13)$ & $-0.29(0.09)$ \\
              & M2-M5 &  15 &  12 & $+2.12(0.04)$ & $-0.39(0.04)$ \\
$\gamma$ Vel  & All K &   9 &  11 & $-2.47(0.02)$ & $+0.41(0.07)$ \\
              & K0-K5 &   6 &   6 & $-1.96(0.08)$ & $+0.42(0.18)$ \\
              & M0-M2 &   5 &   3 & $-2.63(0.04)$ & $+0.67(0.07)$ \\
NGC 2547      & All K &   8 &   9 & $-2.14(0.04)$ & $+0.51(0.04)$ \\
              & K0-K5 &   5 &   9 & $-2.57(0.02)$ & $+0.53(0.05)$ \\
NGC 2516      & All K &  60 & 102 & $-3.96^{*}$ & $+0.29^{*}$ \\
              & K0-K5 &  28 &  55 & $-4.38^{*}$ & $+0.36^{*}$ \\
              & K5-M0 &  32 &  47 & $-1.59(0.12)$ & $+0.22(0.06)$ \\
              & M0-M2 &  33 &  27 & $-1.68(0.10)$ & $+0.20(0.13)$ \\
%
%NGC 2547      & K0-K5 & 17 &  30 & $-0.230$ & $0.119$ \\
%              & K5-M0 & 22 &  13 & $+0.225$ & $0.194$ \\
%              & M0-M2 & 19 &  22 & $+0.267$ & $0.092$ \\
%$\lambda$ Ori & All K &  9 &  12 & $+0.356$ & $0.113$ \\
%              & K0-K5 &  7 &  10 & $+0.363$ & $0.152$ \\
%              & All M & 19 &  17 & $-0.285$ & $0.092$ \\
%              & M0-M2 &  4 &   5 & $+0.517$ & $0.154$ \\
%              & M2-M5 & 15 &  12 & $-0.392$ & $0.043$ \\
%$\gamma$ Vel  & All K &  9 &  11 & $+0.411$ & $0.072$ \\
%              & K0-K5 &  6 &   6 & $+0.420$ & $0.175$ \\
%              & M0-M2 &  5 &   3 & $+0.667$ & $0.071$ \\
%NGC 2547      & All K &  8 &   9 & $+0.507$ & $0.038$ \\
%              & K0-K5 &  5 &   9 & $+0.530$ & $0.051$ \\
%              & K5-M0 &  3 &   1 & $-1.000$ & $0.000$ \\
%NGC 2516      & All K & 60 & 102 & $+0.286$ & $2.2e-4$ \\
%              & K0-K5 & 28 &  55 & $+0.360$ & $0.001$ \\
%              & K5-M0 & 32 &  47 & $+0.217$ & $0.055$ \\
%              & All M & 48 &  46 & $+0.143$ & $0.170$ \\
%              & M0-M2 & 33 &  27 & $+0.197$ & $0.131$ \\
\hline
\end{tabular}
\label{T_CMD_Student}
\end{center}
\end{table}}

==> t_EWLi_StudentT.tex <==
{\centering
\begin{table}
\caption{Results for the statistical tests comparing the $P_{\rm rot}$ distributions between Li-rich and Li-poor samples amongst K- and M-stars in each cluster. Columns 2 and 3 indicate the number of objects in the Li-rich and Li-poor sample, respectively. The Student t-statistic in column 4 represents the difference in the means between the Li-rich and Li-poor populations, where the p-values (that they have significantly different means) are provided in parentheses. Column 5 gives the correlation coefficients (r-scores) for $P_{\rm rot}$ versus $\delta$EW(Li) for the K-stars and $P_{\rm rot}$ versus EW(Li) for the M-stars, with corresponding p-values in parentheses. Asterisks denote p-values that are at least 10 times smaller than 0.01 (highly significant).}
\begin{center}
\begin{tabular}{p{1.35cm}p{0.40cm}p{0.40cm}p{1.30cm}p{1.40cm}}
%\begin{tabular}{llrrrr}
\hline
\hline
Cluster       & R  & P  & t-score  & r-score \\
\hline
\multicolumn{5}{c}{K stars} \\
\hline
NGC~2264      & 51 & 18 & $-0.95(0.35)$ & $-0.05(0.68)$ \\
$\lambda$ Ori & 11 & 5  & $-0.44(0.67)$ & $+0.01(0.97)$ \\
$\gamma$ Vel  & 16 & 2  &               & $-0.14(0.57)$ \\
NGC~2547      & 10 & 7  & $-3.06(0.01)$ & $-0.57(0.02)$ \\
NGC~2516      & 66 & 96 & $-3.75^{*}$   & $-0.34^{*}$ \\
\hline
\multicolumn{5}{c}{M stars} \\
\hline
NGC~2264      & 48 & 38 & $-0.52(0.60)$ & $-0.04(0.71)$ \\
$\lambda$ Ori & 15 & 12 & $+1.13(0.27)$ & $+0.05(0.79)$ \\
$\gamma$ Vel  & 9  & 10 & $+3.22(0.01)$ & $+0.41(0.08)$ \\
%
%$\lambda$ Ori & K0-K5 &  3 &  6 & $-1.85$ & $0.11$ \\ 0.2362637      0.437
%              & M2-M5 & 12 & 10 & $+1.33$ & $0.20$ \\
%$\gamma$ Vel  & All M &  8 &  6 & $+1.88$ & $0.08$ \\
%NGC 2547      & All K &  8 &  6 & $-4.72$ & $4.95$e$-4$ \\
%              & K0-K5 &  5 &  5 & $-3.31$ & $0.01$ \\
%NGC 2516      & K     & 60 & 95 & $-3.59$ & $4.44$e$-4$ \\
%              & K0-K5 & 34 & 49 & $-4.77$ & $8.11$e$-6$ \\
%
%$\lambda$ Ori & K5-M0 &  1 &  2 & $+1.000$ & $0.000$ \\
%$\gamma$ Vel  & All M & 10 &  6 & $+0.374$ & $0.154$ \\
%              & M0-M2 &  4 &  1 & $+0.800$ & $0.104$ \\
%NGC 2547      & All K &  9 &  7 & $-0.803$ & $1.8e-4$ \\
%              & K0-K5 &  7 &  6 & $-0.797$ & $0.001$ \\
%NGC 2516      & All K & 60 & 95 & $-0.349$ & $8.4e-6$ \\
%              & K0-K5 & 34 & 49 & $-0.477$ & $5.0e-6$ \\
%              & K5-M0 & 26 & 46 & $-0.197$ & $0.097$ \\
\hline
\end{tabular}
\label{T_EWLi_GKs_Student}
\end{center}
\end{table}}
